Survey on Characterizing and Understanding GNNs from a Computer Architecture Perspective

Characterizing and understanding graph neural networks (GNNs) is essential for identifying performance bottlenecks and facilitating their deployment in parallel and distributed systems. Despite substantial work in this area, a comprehensive survey on characterizing and understanding GNNs from a computer architecture perspective is lacking. This work presents a comprehensive survey, proposing a triple-level classification method to categorize, summarize, and compare existing efforts, particularly focusing on their implications for parallel architectures and distributed systems. We identify promising future directions for GNN characterization that align with the challenges of optimizing hardware and software in parallel and distributed systems. Our survey aims to help scholars systematically understand GNN performance bottlenecks and execution patterns from a computer architecture perspective, thereby contributing to the development of more efficient GNN implementations across diverse parallel architectures and distributed systems.

==> tex/simple_bio.tex <==
\section{Biography Section}

\renewenvironment{IEEEbiography}[1]
  {\IEEEbiographynophoto{#1}}
  {\endIEEEbiographynophoto}
  
\begin{IEEEbiography}{Meng Wu} received the M.Eng. degree from University of Chinese Academy of Sciences, Beijing, China, in 2017. She is currently working toward the Ph.D. degree at Institute of Computing Technology, Chinese Academy of Sciences, Beijing, China. Her current research interests include graph-based hardware accelerator, high-throughput computer architecture, and parallel algorithm. %To date, she has published over 10 research papers in compute journals and conferences, including IEEE TPDS, FCGS, IEEE CAL, J INF SCI, NOCS, Euro-Par and so on.
\end{IEEEbiography}

\begin{IEEEbiography}{Mingyu Yan} received the Ph.D. degree from University of Chinese Academy of Sciences, Beijing, China in 2020. He is currently an Associate Professor at Institute of Computing Technology, Chinese Academy of Sciences, Beijing, China. His current research interests is domain-specific hardware architecture for graph-based machine learning. %To date, Dr. Yan has published over 20 research papers in top-tier journals and conferences, including the MICRO, HPCA, AAAI, IJCAI, DAC, ICCAD, PIEEE, IEEE TPDS, IEEE TC, IEEE TCAD, IEEE/CAA JAS, IEEE J-STSP, and so on. He has served as the TPC or ERC member for ISCA, HPCA, MICRO, and ICS.

\end{IEEEbiography}


\begin{IEEEbiography}{Wenming Li}
received the Ph.D. degree in computer architecture from Institute of Computing Technology, Chinese Academy of Sciences, Beijing, in 2016. He is currently an associate professor in Institute of Computing Technology, Chinese Academy of Sciences, Beijing. His main research interests include high-throughput processor architecture, dataflow architecture and software simulation. %To date, Dr. Li has published over 30 research papers in compute journals and conferences, including the HPCA, DAC, IEEE TC, IEEE TPDS, IEEE TACO, IEEE TCAD, and so on. 

\end{IEEEbiography}



\begin{IEEEbiography}{Xiaochun Ye} received the Ph.D. degree in computer architecture from Institute of Computing Technology, Chinese Academy of Sciences, Beijing, in 2010. 
He is currently a Professor at Institute of Computing Technology, Chinese Academy of
Sciences, Beijing. 
His main research interest is domain-specific hardware architecture for graph-based machine learning and high-throughput computer architecture.
%To date, Dr. Ye has published over 90 research papers in compute journals and conferences, the MICRO, HPCA, PACT, IPDPS, PIEEE, IEEE TC, IEEE TPDS, IEEE TACO, etc. 


\end{IEEEbiography}

\begin{IEEEbiography}{Dongrui Fan} received the Ph.D. degree in computer architecture from Institute of Computing Technology, Chinese Academy of Sciences, Beijing, in 2005. 
He is currently a Professor and Ph.D. Supervisor at Institute of Computing Technology, Chinese Academy of Sciences, Beijing. 
His main research interests include high-throughput computer architecture and high-performance computer architecture.
%To date, Dr. Fan has published over 140 research papers in compute journals and conferences, including the MICRO, HPCA, PPoPP, IJCAI, PACT, PIEEE, IEEE TC, IEEE TPDS, IEEE TCAD, IEEE TACO, IEEE Micro, and so on. He has been a member of the program committee of many important academic conferences, including MICRO, HPCA, etc.

\end{IEEEbiography}



\begin{IEEEbiography}{Yuan Xie} (Fellow, IEEE) received the B.S. degree in electronic engineering from Tsinghua University, Beijing, China, in 1997, and the M.S. and Ph.D. degrees in electrical engineering from Princeton University, Princeton, NJ, USA, in 1999 and 2002, respectively. He has a rich industry experience with IBM, AMD, and Alibaba Group. He was also on the faculty of Pennsylvania State University and University of California, Santa Barbara. He is a Fellow of IEEE, a Fellow of ACM, and a Fellow of AAAS. 
He is currently a Professor with the Department of Electrical and Computer Engineering, Hong Kong University of Science and Technology, Hong Kong, SAR, China. 
His research interests include VLSI design, electronics design automation (EDA), computer architecture, and embedded systems.

\end{IEEEbiography}
